Graph Domain Adaptation Does Not End with Representation Learning

Graph domain adaptation (GDA) transfers knowledge from a labeled source graph to an unlabeled target graph under shifts in both node attributes and graph structure. Existing methods primarily adapt graph representations through propagation redesign, distribution alignment, or source-to-target transition modeling, but still rely on a single graph-propagating path for target prediction. This leaves open whether an adapted graph representation exhausts the predictive evidence available in the target domain, since the graph-aware expert and graph-free local expert may exhibit different failure modes under topological shifts. To address this limitation, we propose EviGDA, an Evidence-Augmented Graph Domain Adaptation framework that complements graph representation adaptation with a graph-free local expert. The graph-aware expert performs message passing and entropy-aware marginal alignment, while the graph-free local expert learns solely from source node features and labels without graph propagation or target alignment. The two experts are optimized independently and combined only at inference through a task-level constant probability mixture, preserving complementary evidence without joint training, learned routing, or target pseudo-labels. Extensive experiments on ten datasets and 16 transfer tasks show that EviGDA outperforms state-of-the-art baselines. Complementary prediction paths add value beyond graph representation alignment.

==> authors.tex <==
% Public preprint: affiliations and contribution notes in the first-page footnote.
\author{Ziqian Liu \and Yongxue Xu \and Enze Zhang \and Jiaqi Zhang \and Hao Wang \and Maolin Wang}
\makeatletter
\renewcommand{\maketitle}{%
  \begingroup
  \centering
  {\LARGE\bfseries Graph Domain Adaptation Does Not End\\[3pt]
  with Representation Learning\par}
  \vspace{15pt}
  {\large\normalfont
  Ziqian Liu\textsuperscript{1,*}\qquad
  Yongxue Xu\textsuperscript{1,*}\qquad
  Enze Zhang\textsuperscript{2}\\[5pt]
  Jiaqi Zhang\textsuperscript{3}\qquad
  Hao Wang\textsuperscript{4}\qquad
  Maolin Wang\textsuperscript{5,\ensuremath{\dagger}}\par}
  \vspace{13pt}
  \endgroup
  \begingroup
  \renewcommand{\thefootnote}{}%
  \renewcommand{\@makefntext}[1]{\noindent##1}%
  \footnotetext{%
  \textsuperscript{1}Sun Yat-sen University, China.
  \textsuperscript{2}University of Wisconsin--Madison, USA.\newline
  \textsuperscript{3}Jiangsu University, China.
  \textsuperscript{4}Zhejiang University, China.
  \textsuperscript{5}City University of Hong Kong, China.\newline
  \textsuperscript{*}Equal contribution.
  \textsuperscript{\ensuremath{\dagger}}Corresponding author: Maolin Wang.}
  \endgroup
  \setcounter{footnote}{0}%
}
\makeatother


